Search for the decay $B^{0}\to\gamma\gamma$ using Belle and Belle II data

We report the result of a search for the rare decay $B^{0} \to \gamma \gamma$ using a combined dataset of $753\times10^{6}$ $B\bar{B}$ pairs collected by the Belle experiment and $387\times10^{6}$ $B\bar{B}$ pairs collected by the Belle II experiment from decays of the $\rm \Upsilon(4S)$ resonance produced in $e^{+}e^{-}$ collisions. A simultaneous fit to the Belle and Belle II data sets yields $11.0^{+6.5}_{-5.5}$ signal events, corresponding to a 2.5$\sigma$ significance. We determine the branching fraction $\mathcal{B}(B^{0} \to \gamma\gamma) = (3.7^{+2.2}_{-1.8}(\rm stat)\pm0.5(\rm syst))\times10^{-8}$ and set a 90% credibility level upper limit of $\mathcal{B}(B^{0} \to \gamma\gamma) < 6.4\times10^{-8}$.

==> acknowledgements.tex <==
% Policy from October 20, 2022
This work, based on data collected using the Belle II detector, which was built and commissioned prior to March 2019,
and data collected using the Belle detector, which was operated until June 2010,
was supported by
%Armenia
Higher Education and Science Committee of the Republic of Armenia Grant No.~23LCG-1C011;
%Australia
Australian Research Council and Research Grants
No.~DP200101792, % Jackson
No.~DP210101900, % Urquijo
No.~DP210102831, % Sevior
No.~DE220100462, % Hsu
No.~LE210100098, % Infrastructure
and
No.~LE230100085; % Infrastructure
%Austria
Austrian Federal Ministry of Education, Science and Research,
Austrian Science Fund
No.~P~34529,
No.~J~4731,
No.~J~4625,
and
No.~M~3153,
and
Horizon 2020 ERC Starting Grant No.~947006 ``InterLeptons'';
%Canada
Natural Sciences and Engineering Research Council of Canada, Compute Canada and CANARIE;
%China
National Key R\&D Program of China under Contract No.~2022YFA1601903,
National Natural Science Foundation of China and Research Grants
No.~11575017,
No.~11761141009,
No.~11705209,
No.~11975076,
No.~12135005,
No.~12150004,
No.~12161141008,
and
No.~12175041,
and Shandong Provincial Natural Science Foundation Project~ZR2022JQ02;
%Czech Republic
the Czech Science Foundation Grant No.~22-18469S 
and
Charles University Grant Agency project No.~246122;
%EU
European Research Council, Seventh Framework PIEF-GA-2013-622527,
Horizon 2020 ERC-Advanced Grants No.~267104 and No.~884719,
Horizon 2020 ERC-Consolidator Grant No.~819127,
Horizon 2020 Marie Sklodowska-Curie Grant Agreement No.~700525 ``NIOBE''
and
No.~101026516,
and
Horizon 2020 Marie Sklodowska-Curie RISE project JENNIFER2 Grant Agreement No.~822070 (European grants);
%France
L'Institut National de Physique Nucl\'{e}aire et de Physique des Particules (IN2P3) du CNRS
and
L'Agence Nationale de la Recherche (ANR) under grant ANR-21-CE31-0009 (France);
%Germany
BMBF, DFG, HGF, MPG, and AvH Foundation (Germany);
%India
Department of Atomic Energy under Project Identification No.~RTI 4002,
Department of Science and Technology,
and
UPES SEED funding programs
No.~UPES/R\&D-SEED-INFRA/17052023/01 and
No.~UPES/R\&D-SOE/20062022/06 (India);
%Israel
Israel Science Foundation Grant No.~2476/17,
U.S.-Israel Binational Science Foundation Grant No.~2016113, and
Israel Ministry of Science Grant No.~3-16543;
%Italy
Istituto Nazionale di Fisica Nucleare and the Research Grants BELLE2;
%Japan
Japan Society for the Promotion of Science, Grant-in-Aid for Scientific Research Grants
No.~16H03968,
No.~16H03993,
No.~16H06492,
No.~16K05323,
No.~17H01133,
No.~17H05405,
No.~18K03621,
No.~18H03710,
No.~18H05226,
No.~19H00682, % Niigata
No.~20H05850,
No.~20H05858,
No.~22H00144,
No.~22K14056,
No.~22K21347,
No.~23H05433,
No.~26220706,
and
No.~26400255,
%the National Institute of Informatics, and Science Information NETwork 5 (SINET5), 
and
the Ministry of Education, Culture, Sports, Science, and Technology (MEXT) of Japan;  
%Korea
National Research Foundation (NRF) of Korea Grants
No.~2016R1\-D1A1B\-02012900,
No.~2018R1\-A2B\-3003643,
No.~2018R1\-A6A1A\-06024970,
No.~2019R1\-I1A3A\-01058933,
No.~2021R1\-A6A1A\-03043957,
No.~2021R1\-F1A\-1060423,
No.~2021R1\-F1A\-1064008,
No.~2022R1\-A2C\-1003993,
and
No.~RS-2022-00197659,
Radiation Science Research Institute,
Foreign Large-Size Research Facility Application Supporting project,
the Global Science Experimental Data Hub Center of the Korea Institute of Science and Technology Information
and
KREONET/GLORIAD;
%Malaysia
Universiti Malaya RU grant, Akademi Sains Malaysia, and Ministry of Education Malaysia;
%Mexico
% CINVESTAV-IPN, UNAM, UAS, BUAP and CONACYT are funded under
Frontiers of Science Program Contracts
No.~FOINS-296,
No.~CB-221329,
No.~CB-236394,
No.~CB-254409,
and
No.~CB-180023, and SEP-CINVESTAV Research Grant No.~237 (Mexico);
%Poland
the Polish Ministry of Science and Higher Education and the National Science Center;
%Russia
the Ministry of Science and Higher Education of the Russian Federation
and
the HSE University Basic Research Program, Moscow;
%Saudi Arabia
University of Tabuk Research Grants
No.~S-0256-1438 and No.~S-0280-1439 (Saudi Arabia);
%Slovenia
Slovenian Research Agency and Research Grants
No.~J1-9124
and
No.~P1-0135;
%Spain
Ikerbasque, Basque Foundation for Science,
the State Agency for Research of the Spanish Ministry of Science and Innovation through Grant No. PID2022-136510NB-C33,
Agencia Estatal de Investigacion, Spain
Grant No.~RYC2020-029875-I
and
Generalitat Valenciana, Spain
Grant No.~CIDEGENT/2018/020;
%Swiss (Belle 1)
the Swiss National Science Foundation;
%Sweden
The Knut and Alice Wallenberg Foundation (Sweden), Contracts No.~2021.0174 and No.~2021.0299;
%Taiwan
National Science and Technology Council,
and
Ministry of Education (Taiwan);
%Thailand
Thailand Center of Excellence in Physics;
%Turkey
TUBITAK ULAKBIM (Turkey);
%Ukraine
National Research Foundation of Ukraine, Project No.~2020.02/0257,
and
Ministry of Education and Science of Ukraine;
%USA
the U.S. National Science Foundation and Research Grants
No.~PHY-1913789 % Indiana CEEM
and
No.~PHY-2111604, % Luther
and the U.S. Department of Energy and Research Awards
No.~DE-AC06-76RLO1830, % PNNL
No.~DE-SC0007983, % Wayne State
No.~DE-SC0009824, % Florida
No.~DE-SC0009973, % VPI
No.~DE-SC0010007, % Duke
No.~DE-SC0010073, % South Carolina
No.~DE-SC0010118, % Carnegie Mellon
No.~DE-SC0010504, % Hawaii
No.~DE-SC0011784, % Cincinnati
No.~DE-SC0012704, % BNL
No.~DE-SC0019230, % Duke
No.~DE-SC0021274, % Mississippi
No.~DE-SC0021616, % Mississippi
No.~DE-SC0022350, % Louisville
No.~DE-SC0023470; % South Alabama
%last group
and
%Vietnam
the Vietnam Academy of Science and Technology (VAST) under Grants
No.~NVCC.05.12/22-23
and
No.~DL0000.02/24-25.

% Policy from October 20, 2022
These acknowledgements are not to be interpreted as an endorsement of any statement made
by any of our institutes, funding agencies, governments, or their representatives.

We thank the SuperKEKB team for delivering high-luminosity collisions;
the KEK cryogenics group for the efficient operation of the detector solenoid magnet;
the KEK Computer Research Center for on-site computing support; the NII for SINET6 network support;
and the raw-data centers hosted by BNL, DESY, GridKa, IN2P3, INFN, 
PNNL/EMSL, 
and the University of Victoria.


==> authors.tex <==
%%% Paper:    B0 to gamma gamma
%%% Journal:  Physical Review D Letter
%%% Contacts: S.K. Maurya, D. Kalita, B. Bhuyan
%%% ====================================================================
%%% Use \input{pub051-orcid} to insert this material into your latex file.
  \author{I.~Adachi\,\orcidlink{0000-0003-2287-0173}} % 2590
% \author{K.~Adamczyk\,\orcidlink{0000-0001-6208-0876}} % 2239
  \author{L.~Aggarwal\,\orcidlink{0000-0002-0909-7537}} % 10083
% \author{P.~Ahlburg\,\orcidlink{0000-0002-9832-7604}} % 2367
% \author{H.~Ahmed\,\orcidlink{0000-0003-3976-7498}} % 11323
% \author{J.~K.~Ahn\,\orcidlink{0000-0002-5795-2243}} % 7423
  \author{H.~Aihara\,\orcidlink{0000-0002-1907-5964}} % 2223
  \author{N.~Akopov\,\orcidlink{0000-0002-4425-2096}} % 9443
  \author{A.~Aloisio\,\orcidlink{0000-0002-3883-6693}} % 2194
  \author{S.~Al~Said\,\orcidlink{0000-0002-4895-3869}} % 6823
  \author{N.~Althubiti\,\orcidlink{0000-0003-1513-0409}} % 21524
% \author{L.~Andricek\,\orcidlink{0000-0003-1755-4475}} % 2098
% \author{M.~Angelsmark\,\orcidlink{0000-0003-4745-1020}} % 13963
  \author{N.~Anh~Ky\,\orcidlink{0000-0003-0471-197X}} % 2218
  \author{D.~M.~Asner\,\orcidlink{0000-0002-1586-5790}} % 4684
  \author{H.~Atmacan\,\orcidlink{0000-0003-2435-501X}} % 2538
% \author{V.~Aulchenko\,\orcidlink{0000-0002-5394-4406}} % 8183
  \author{T.~Aushev\,\orcidlink{0000-0002-6347-7055}} % 3747
  \author{V.~Aushev\,\orcidlink{0000-0002-8588-5308}} % 2155
  \author{M.~Aversano\,\orcidlink{0000-0001-9980-0953}} % 7363
  \author{R.~Ayad\,\orcidlink{0000-0003-3466-9290}} % 3766
% \author{T.~Aziz\,\orcidlink{-}} % 3523
  \author{V.~Babu\,\orcidlink{0000-0003-0419-6912}} % 5623
% \author{S.~Bacher\,\orcidlink{0000-0002-2656-2330}} % 2258
  \author{H.~Bae\,\orcidlink{0000-0003-1393-8631}} % 10863
  \author{S.~Bahinipati\,\orcidlink{0000-0002-3744-5332}} % 2332
% \author{A.~M.~Bakich\,\orcidlink{0000-0001-8315-4854}} % 2115
  \author{P.~Bambade\,\orcidlink{0000-0001-7378-4852}} % 3003
  \author{Sw.~Banerjee\,\orcidlink{0000-0001-8852-2409}} % 8603
  \author{S.~Bansal\,\orcidlink{0000-0003-1992-0336}} % 5163
  \author{M.~Barrett\,\orcidlink{0000-0002-2095-603X}} % 2180
% \author{G.~Batignani\,\orcidlink{0000-0003-3917-3104}} % 6643
  \author{J.~Baudot\,\orcidlink{0000-0001-5585-0991}} % 2562
% \author{M.~Bauer\,\orcidlink{0000-0002-0953-7387}} % 9863
  \author{A.~Baur\,\orcidlink{0000-0003-1360-3292}} % 5683
  \author{A.~Beaubien\,\orcidlink{0000-0001-9438-089X}} % 6683
  \author{F.~Becherer\,\orcidlink{0000-0003-0562-4616}} % 21623
  \author{J.~Becker\,\orcidlink{0000-0002-5082-5487}} % 5403
% \author{P.~K.~Behera\,\orcidlink{0000-0002-1527-2266}} % 4204
  \author{K.~Belous\,\orcidlink{0000-0003-0014-2589}} % 2329
  \author{J.~V.~Bennett\,\orcidlink{0000-0002-5440-2668}} % 2454
% \author{E.~Bernieri\,\orcidlink{0000-0002-4787-2047}} % 4483
  \author{F.~U.~Bernlochner\,\orcidlink{0000-0001-8153-2719}} % 2282
  \author{V.~Bertacchi\,\orcidlink{0000-0001-9971-1176}} % 2212
% \author{M.~Bertemes\,\orcidlink{0000-0001-5038-360X}} % 2595
  \author{E.~Bertholet\,\orcidlink{0000-0002-3792-2450}} % 13163
  \author{M.~Bessner\,\orcidlink{0000-0003-1776-0439}} % 3783
% \author{D.~Besson\,\orcidlink{-}} % 3585
  \author{S.~Bettarini\,\orcidlink{0000-0001-7742-2998}} % 2350
% \author{V.~Bhardwaj\,\orcidlink{0000-0001-8857-8621}} % 2228
  \author{B.~Bhuyan\,\orcidlink{0000-0001-6254-3594}} % 2097
  \author{F.~Bianchi\,\orcidlink{0000-0002-1524-6236}} % 2564
  \author{L.~Bierwirth\,\orcidlink{0009-0003-0192-9073}} % 11723
  \author{T.~Bilka\,\orcidlink{0000-0003-1449-6986}} % 2484
% \author{S.~Bilokin\,\orcidlink{0000-0003-0017-6260}} % 3623
  \author{D.~Biswas\,\orcidlink{0000-0002-7543-3471}} % 8703
% \author{T.~Bloomfield\,\orcidlink{0000-0001-9288-5069}} % 2418
  \author{A.~Bobrov\,\orcidlink{0000-0001-5735-8386}} % 2294
  \author{D.~Bodrov\,\orcidlink{0000-0001-5279-4787}} % 9643
  \author{A.~Bolz\,\orcidlink{0000-0002-4033-9223}} % 15403
% \author{A.~Bondar\,\orcidlink{0000-0002-5089-5338}} % 4643
% \author{G.~Bonvicini\,\orcidlink{0000-0003-4861-7918}} % 2095
  \author{J.~Borah\,\orcidlink{0000-0003-2990-1913}} % 7083
  \author{A.~Boschetti\,\orcidlink{0000-0001-6030-3087}} % 17683
  \author{A.~Bozek\,\orcidlink{0000-0002-5915-1319}} % 2303
  \author{M.~Bra\v{c}ko\,\orcidlink{0000-0002-2495-0524}} % 2425
  \author{P.~Branchini\,\orcidlink{0000-0002-2270-9673}} % 2577
% \author{N.~Brenny\,\orcidlink{0009-0006-2917-9173}} % 19943
  \author{R.~A.~Briere\,\orcidlink{0000-0001-5229-1039}} % 2584
  \author{T.~E.~Browder\,\orcidlink{0000-0001-7357-9007}} % 2560
% \author{Y.~Buch\,\orcidlink{0000-0002-8050-4000}} % 17323
  \author{A.~Budano\,\orcidlink{0000-0002-0856-1131}} % 2171
  \author{S.~Bussino\,\orcidlink{0000-0002-3829-9592}} % 5384
% \author{A.~Calcaterra\,\orcidlink{0000-0003-2670-4826}} % 19163
  \author{Q.~Campagna\,\orcidlink{0000-0002-3109-2046}} % 21563
  \author{M.~Campajola\,\orcidlink{0000-0003-2518-7134}} % 5223
  \author{L.~Cao\,\orcidlink{0000-0001-8332-5668}} % 2099
  \author{G.~Casarosa\,\orcidlink{0000-0003-4137-938X}} % 2491
  \author{C.~Cecchi\,\orcidlink{0000-0002-2192-8233}} % 2433
  \author{J.~Cerasoli\,\orcidlink{0000-0001-9777-881X}} % 20746
  \author{M.-C.~Chang\,\orcidlink{0000-0002-8650-6058}} % 2827
  \author{P.~Chang\,\orcidlink{0000-0003-4064-388X}} % 2542
% \author{R.~Cheaib\,\orcidlink{0000-0001-5729-8926}} % 2208
  \author{P.~Cheema\,\orcidlink{0000-0001-8472-5727}} % 15264
% \author{V.~Chekelian\,\orcidlink{0000-0001-8860-8288}} % 2167
  \author{C.~Chen\,\orcidlink{0000-0003-1589-9955}} % 12803
% \author{Y.~Q.~Chen\,\orcidlink{0000-0002-7285-3251}} % 16264
% \author{Y.-T.~Chen\,\orcidlink{0000-0003-2639-2850}} % 2884
  \author{B.~G.~Cheon\,\orcidlink{0000-0002-8803-4429}} % 2173
  \author{K.~Chilikin\,\orcidlink{0000-0001-7620-2053}} % 2308
  \author{K.~Chirapatpimol\,\orcidlink{0000-0003-2099-7760}} % 10803
  \author{H.-E.~Cho\,\orcidlink{0000-0002-7008-3759}} % 2182
  \author{K.~Cho\,\orcidlink{0000-0003-1705-7399}} % 2516
  \author{S.-J.~Cho\,\orcidlink{0000-0002-1673-5664}} % 2723
  \author{S.-K.~Choi\,\orcidlink{0000-0003-2747-8277}} % 2364
  \author{S.~Choudhury\,\orcidlink{0000-0001-9841-0216}} % 2206
% \author{D.~Cinabro\,\orcidlink{0000-0001-7347-6585}} % 2092
% \author{J.~Cochran\,\orcidlink{0000-0002-1492-914X}} % 12604
  \author{L.~Corona\,\orcidlink{0000-0002-2577-9909}} % 3944
% \author{L.~M.~Cremaldi\,\orcidlink{0000-0001-5550-7827}} % 2276
  \author{J.~X.~Cui\,\orcidlink{0000-0002-2398-3754}} % 8863
% \author{T.~Czank\,\orcidlink{0000-0001-6621-3373}} % 2254
% \author{S.~Das\,\orcidlink{0000-0001-6857-966X}} % 9163
  \author{F.~Dattola\,\orcidlink{0000-0003-3316-8574}} % 3745
  \author{E.~De~La~Cruz-Burelo\,\orcidlink{0000-0002-7469-6974}} % 2359
  \author{S.~A.~De~La~Motte\,\orcidlink{0000-0003-3905-6805}} % 2128
% \author{G.~de~Marino\,\orcidlink{0000-0002-6509-7793}} % 8364
  \author{G.~De~Nardo\,\orcidlink{0000-0002-2047-9675}} % 2459
  \author{M.~De~Nuccio\,\orcidlink{0000-0002-0972-9047}} % 2610
  \author{G.~De~Pietro\,\orcidlink{0000-0001-8442-107X}} % 2528
  \author{R.~de~Sangro\,\orcidlink{0000-0002-3808-5455}} % 2524
% \author{B.~Deschamps\,\orcidlink{0000-0003-2497-5008}} % 2671
  \author{M.~Destefanis\,\orcidlink{0000-0003-1997-6751}} % 2594
  \author{S.~Dey\,\orcidlink{0000-0003-2997-3829}} % 5023
% \author{A.~De~Yta-Hernandez\,\orcidlink{0000-0002-2162-7334}} % 2104
  \author{R.~Dhamija\,\orcidlink{0000-0001-7052-3163}} % 9465
  \author{A.~Di~Canto\,\orcidlink{0000-0003-1233-3876}} % 10963
  \author{F.~Di~Capua\,\orcidlink{0000-0001-9076-5936}} % 2065
  \author{J.~Dingfelder\,\orcidlink{0000-0001-5767-2121}} % 2151
  \author{Z.~Dole\v{z}al\,\orcidlink{0000-0002-5662-3675}} % 2319
  \author{I.~Dom\'{\i}nguez~Jim\'{e}nez\,\orcidlink{0000-0001-6831-3159}} % 2191
  \author{T.~V.~Dong\,\orcidlink{0000-0003-3043-1939}} % 2215
  \author{M.~Dorigo\,\orcidlink{0000-0002-0681-6946}} % 12543
  \author{D.~Dorner\,\orcidlink{0000-0003-3628-9267}} % 13564
  \author{K.~Dort\,\orcidlink{0000-0003-0849-8774}} % 5583
  \author{D.~Dossett\,\orcidlink{0000-0002-5670-5582}} % 2574
  \author{S.~Dreyer\,\orcidlink{0000-0002-6295-100X}} % 12823
  \author{S.~Dubey\,\orcidlink{0000-0002-1345-0970}} % 11063
% \author{S.~Duell\,\orcidlink{0000-0001-9918-9808}} % 2344
  \author{K.~Dugic\,\orcidlink{0009-0006-6056-546X}} % 11103
  \author{G.~Dujany\,\orcidlink{0000-0002-1345-8163}} % 9703
  \author{P.~Ecker\,\orcidlink{0000-0002-6817-6868}} % 5563
  \author{M.~Eliachevitch\,\orcidlink{0000-0003-2033-537X}} % 2725
  \author{D.~Epifanov\,\orcidlink{0000-0001-8656-2693}} % 2551
% \author{Y.~Fan\,\orcidlink{0000-0001-9616-9705}} % 21303
  \author{P.~Feichtinger\,\orcidlink{0000-0003-3966-7497}} % 9843
  \author{T.~Ferber\,\orcidlink{0000-0002-6849-0427}} % 2482
% \author{D.~Ferlewicz\,\orcidlink{0000-0002-4374-1234}} % 2073
  \author{T.~Fillinger\,\orcidlink{0000-0001-9795-7412}} % 9803
  \author{C.~Finck\,\orcidlink{0000-0002-5068-5453}} % 15803
  \author{G.~Finocchiaro\,\orcidlink{0000-0002-3936-2151}} % 2400
% \author{P.~Fischer\,\orcidlink{0000-0002-9808-3574}} % 2141
% \author{K.~Flood\,\orcidlink{0000-0002-3463-6571}} % 12103
  \author{A.~Fodor\,\orcidlink{0000-0002-2821-759X}} % 2312
  \author{F.~Forti\,\orcidlink{0000-0001-6535-7965}} % 2432
  \author{A.~Frey\,\orcidlink{0000-0001-7470-3874}} % 2150
% \author{M.~Friedl\,\orcidlink{0000-0002-7420-2559}} % 2442
  \author{B.~G.~Fulsom\,\orcidlink{0000-0002-5862-9739}} % 2563
% \author{A.~Gabrielli\,\orcidlink{0000-0001-7695-0537}} % 13523
% \author{N.~Gabyshev\,\orcidlink{0000-0002-8593-6857}} % 2510
  \author{E.~Ganiev\,\orcidlink{0000-0001-8346-8597}} % 4623
  \author{M.~Garcia-Hernandez\,\orcidlink{0000-0003-2393-3367}} % 4823
% \author{R.~Garg\,\orcidlink{0000-0002-7406-4707}} % 2213
% \author{A.~Garmash\,\orcidlink{0000-0003-2599-1405}} % 2161
  \author{G.~Gaudino\,\orcidlink{0000-0001-5983-1552}} % 16563
  \author{V.~Gaur\,\orcidlink{0000-0002-8880-6134}} % 2413
  \author{A.~Gaz\,\orcidlink{0000-0001-6754-3315}} % 2181
% \author{U.~Gebauer\,\orcidlink{0000-0002-5679-2209}} % 2174
  \author{A.~Gellrich\,\orcidlink{0000-0003-0974-6231}} % 2480
  \author{G.~Ghevondyan\,\orcidlink{0000-0003-0096-3555}} % 9445
  \author{D.~Ghosh\,\orcidlink{0000-0002-3458-9824}} % 11923
  \author{H.~Ghumaryan\,\orcidlink{0000-0001-6775-8893}} % 19543
  \author{G.~Giakoustidis\,\orcidlink{0000-0001-5982-1784}} % 13723
  \author{R.~Giordano\,\orcidlink{0000-0002-5496-7247}} % 2103
  \author{A.~Giri\,\orcidlink{0000-0002-8895-0128}} % 2106
  \author{A.~Glazov\,\orcidlink{0000-0002-8553-7338}} % 2473
  \author{B.~Gobbo\,\orcidlink{0000-0002-3147-4562}} % 2109
  \author{R.~Godang\,\orcidlink{0000-0002-8317-0579}} % 2449
  \author{O.~Gogota\,\orcidlink{0000-0003-4108-7256}} % 2334
  \author{P.~Goldenzweig\,\orcidlink{0000-0001-8785-847X}} % 2345
% \author{B.~Golob\,\orcidlink{0000-0001-9632-5616}} % 3703
% \author{G.~Gong\,\orcidlink{0000-0001-7192-1833}} % 2727
% \author{P.~Grace\,\orcidlink{0000-0001-9005-7403}} % 9563
  \author{W.~Gradl\,\orcidlink{0000-0002-9974-8320}} % 2570
% \author{M.~Graf-Schreiber\,\orcidlink{0000-0003-4613-1041}} % 2730
% \author{T.~Grammatico\,\orcidlink{0000-0002-2818-9744}} % 20623
% \author{S.~Granderath\,\orcidlink{0000-0002-9945-463X}} % 8383
  \author{E.~Graziani\,\orcidlink{0000-0001-8602-5652}} % 2342
  \author{D.~Greenwald\,\orcidlink{0000-0001-6964-8399}} % 2686
  \author{Z.~Gruberov\'{a}\,\orcidlink{0000-0002-5691-1044}} % 8824
  \author{T.~Gu\,\orcidlink{0000-0002-1470-6536}} % 14283
% \author{Y.~Guan\,\orcidlink{0000-0002-5541-2278}} % 2514
  \author{K.~Gudkova\,\orcidlink{0000-0002-5858-3187}} % 10504
  \author{I.~Haide\,\orcidlink{0000-0003-0962-6344}} % 14824
% \author{H.~Haigh\,\orcidlink{0000-0003-1567-0907}} % 16744
% \author{S.~Halder\,\orcidlink{0000-0002-6280-494X}} % 4743
  \author{Y.~Han\,\orcidlink{0000-0001-6775-5932}} % 19663
% \author{K.~Hara\,\orcidlink{0000-0002-5361-1871}} % 2462
  \author{T.~Hara\,\orcidlink{0000-0002-4321-0417}} % 2523
  \author{C.~Harris\,\orcidlink{0000-0003-0448-4244}} % 21383
% \author{O.~Hartbrich\,\orcidlink{0000-0001-7741-4381}} % 2158
  \author{K.~Hayasaka\,\orcidlink{0000-0002-6347-433X}} % 2330
  \author{H.~Hayashii\,\orcidlink{0000-0002-5138-5903}} % 2455
  \author{S.~Hazra\,\orcidlink{0000-0001-6954-9593}} % 7663
  \author{C.~Hearty\,\orcidlink{0000-0001-6568-0252}} % 2450
  \author{M.~T.~Hedges\,\orcidlink{0000-0001-6504-1872}} % 2265
  \author{A.~Heidelbach\,\orcidlink{0000-0002-6663-5469}} % 16923
  \author{I.~Heredia~de~la~Cruz\,\orcidlink{0000-0002-8133-6467}} % 2559
  \author{M.~Hern\'{a}ndez~Villanueva\,\orcidlink{0000-0002-6322-5587}} % 2466
% \author{A.~Hershenhorn\,\orcidlink{0000-0001-8753-5451}} % 2552
  \author{T.~Higuchi\,\orcidlink{0000-0002-7761-3505}} % 2485
% \author{H.~Hirata\,\orcidlink{0000-0001-9005-4616}} % 2070
  \author{M.~Hoek\,\orcidlink{0000-0002-1893-8764}} % 2101
  \author{M.~Hohmann\,\orcidlink{0000-0001-5147-4781}} % 2077
  \author{P.~Horak\,\orcidlink{0000-0001-9979-6501}} % 13583
% \author{T.~Hotta\,\orcidlink{0000-0002-1079-5826}} % 2084
  \author{C.-L.~Hsu\,\orcidlink{0000-0002-1641-430X}} % 2299
% \author{K.~Huang\,\orcidlink{0000-0001-9342-7406}} % 2389
  \author{T.~Humair\,\orcidlink{0000-0002-2922-9779}} % 10643
  \author{T.~Iijima\,\orcidlink{0000-0002-4271-711X}} % 2446
  \author{K.~Inami\,\orcidlink{0000-0003-2765-7072}} % 2323
% \author{G.~Inguglia\,\orcidlink{0000-0003-0331-8279}} % 2500
  \author{N.~Ipsita\,\orcidlink{0000-0002-2927-3366}} % 12223
% \author{J.~Irakkathil~Jabbar\,\orcidlink{0000-0001-7948-1633}} % 7343
  \author{A.~Ishikawa\,\orcidlink{0000-0002-3561-5633}} % 2281
% \author{S.~Ito\,\orcidlink{0000-0003-2737-8145}} % 17463
  \author{R.~Itoh\,\orcidlink{0000-0003-1590-0266}} % 2487
  \author{M.~Iwasaki\,\orcidlink{0000-0002-9402-7559}} % 2360
% \author{Y.~Iwasaki\,\orcidlink{0000-0001-7261-2557}} % 2229
% \author{S.~Iwata\,\orcidlink{0009-0005-5017-8098}} % 4323
  \author{P.~Jackson\,\orcidlink{0000-0002-0847-402X}} % 2255
  \author{W.~W.~Jacobs\,\orcidlink{0000-0002-9996-6336}} % 2322
  \author{D.~E.~Jaffe\,\orcidlink{0000-0003-3122-4384}} % 3663
  \author{E.-J.~Jang\,\orcidlink{0000-0002-1935-9887}} % 6744
% \author{Q.~P.~Ji\,\orcidlink{0000-0003-2963-2565}} % 16243
  \author{S.~Jia\,\orcidlink{0000-0001-8176-8545}} % 2457
  \author{Y.~Jin\,\orcidlink{0000-0002-7323-0830}} % 2105
  \author{A.~Johnson\,\orcidlink{0000-0002-8366-1749}} % 16143
  \author{K.~K.~Joo\,\orcidlink{0000-0002-5515-0087}} % 4224
  \author{H.~Junkerkalefeld\,\orcidlink{0000-0003-3987-9895}} % 12963
% \author{I.~Kadenko\,\orcidlink{0000-0001-8766-4229}} % 3843
% \author{H.~Kakuno\,\orcidlink{0000-0002-9957-6055}} % 2391
% \author{M.~Kaleta\,\orcidlink{0000-0002-2863-5476}} % 5603
  \author{D.~Kalita\,\orcidlink{0000-0003-3054-1222}} % 2220
  \author{A.~B.~Kaliyar\,\orcidlink{0000-0002-2211-619X}} % 7344
  \author{J.~Kandra\,\orcidlink{0000-0001-5635-1000}} % 2541
  \author{K.~H.~Kang\,\orcidlink{0000-0002-6816-0751}} % 2283
  \author{S.~Kang\,\orcidlink{0000-0002-5320-7043}} % 12683
% \author{P.~Kapusta\,\orcidlink{0000-0003-1235-1935}} % 6663
  \author{G.~Karyan\,\orcidlink{0000-0001-5365-3716}} % 2550
% \author{Y.~Kato\,\orcidlink{0000-0001-6314-4288}} % 2549
% \author{H.~Kawai\,\orcidlink{-}} % 4344
  \author{T.~Kawasaki\,\orcidlink{0000-0002-4089-5238}} % 4363
  \author{F.~Keil\,\orcidlink{0000-0002-7278-2860}} % 19523
% \author{C.~Ketter\,\orcidlink{0000-0002-5161-9722}} % 2236
% \author{M.~Khan\,\orcidlink{0000-0002-2168-0872}} % 15644
  \author{C.~Kiesling\,\orcidlink{0000-0002-2209-535X}} % 2168
  \author{C.-H.~Kim\,\orcidlink{0000-0002-5743-7698}} % 2358
  \author{D.~Y.~Kim\,\orcidlink{0000-0001-8125-9070}} % 2315
% \author{H.~J.~Kim\,\orcidlink{0000-0001-9787-4684}} % 4863
  \author{K.-H.~Kim\,\orcidlink{0000-0002-4659-1112}} % 2118
% \author{K.~Kim\,\orcidlink{-}} % 2409
  \author{Y.-K.~Kim\,\orcidlink{0000-0002-9695-8103}} % 2379
% \author{Y.~J.~Kim\,\orcidlink{0000-0001-9511-9634}} % 2403
  \author{H.~Kindo\,\orcidlink{0000-0002-6756-3591}} % 2195
  \author{K.~Kinoshita\,\orcidlink{0000-0001-7175-4182}} % 2318
% \author{C.~Kleinwort\,\orcidlink{0000-0002-9017-9504}} % 2499
  \author{P.~Kody\v{s}\,\orcidlink{0000-0002-8644-2349}} % 2407
  \author{T.~Koga\,\orcidlink{0000-0002-1644-2001}} % 6963
  \author{S.~Kohani\,\orcidlink{0000-0003-3869-6552}} % 9143
  \author{K.~Kojima\,\orcidlink{0000-0002-3638-0266}} % 6363
% \author{T.~Konno\,\orcidlink{0000-0003-2487-8080}} % 2490
% \author{H.~Korandla\,\orcidlink{0000-0003-0516-7793}} % 18783
  \author{A.~Korobov\,\orcidlink{0000-0001-5959-8172}} % 4185
  \author{S.~Korpar\,\orcidlink{0000-0003-0971-0968}} % 2475
% \author{E.~Kou\,\orcidlink{0000-0002-8650-6699}} % 3765
  \author{E.~Kovalenko\,\orcidlink{0000-0001-8084-1931}} % 3884
  \author{R.~Kowalewski\,\orcidlink{0000-0002-7314-0990}} % 2293
% \author{T.~M.~G.~Kraetzschmar\,\orcidlink{0000-0001-8395-2928}} % 7543
  \author{P.~Kri\v{z}an\,\orcidlink{0000-0002-4967-7675}} % 2474
% \author{R.~Kroeger\,\orcidlink{-}} % 2242
% \author{J.~F.~Krohn\,\orcidlink{0000-0002-5001-0675}} % 2502
  \author{P.~Krokovny\,\orcidlink{0000-0002-1236-4667}} % 2575
% \author{W.~Kuehn\,\orcidlink{0000-0001-6018-9878}} % 2534
% \author{M.~K\"{u}nzel\,\orcidlink{-}} % 2139
  \author{T.~Kuhr\,\orcidlink{0000-0001-6251-8049}} % 2486
  \author{Y.~Kulii\,\orcidlink{0000-0001-6217-5162}} % 9823
  \author{J.~Kumar\,\orcidlink{0000-0002-8465-433X}} % 6464
% \author{M.~Kumar\,\orcidlink{0000-0002-6627-9708}} % 2744
  \author{R.~Kumar\,\orcidlink{0000-0002-6277-2626}} % 2189
  \author{K.~Kumara\,\orcidlink{0000-0003-1572-5365}} % 2257
% \author{T.~Kumita\,\orcidlink{0000-0001-7572-4538}} % 4083
  \author{T.~Kunigo\,\orcidlink{0000-0001-9613-2849}} % 10104
% \author{A.~Kusudo\,\orcidlink{0000-0002-2662-9734}} % 14623
  \author{A.~Kuzmin\,\orcidlink{0000-0002-7011-5044}} % 2520
% \author{P.~Kvasni\v{c}ka\,\orcidlink{0000-0001-6281-0648}} % 2184
  \author{Y.-J.~Kwon\,\orcidlink{0000-0001-9448-5691}} % 2231
  \author{S.~Lacaprara\,\orcidlink{0000-0002-0551-7696}} % 2447
% \author{Y.-T.~Lai\,\orcidlink{0000-0001-9553-3421}} % 2066
  \author{K.~Lalwani\,\orcidlink{0000-0002-7294-396X}} % 2142
  \author{T.~Lam\,\orcidlink{0000-0001-9128-6806}} % 2729
% \author{L.~Lanceri\,\orcidlink{0000-0001-8220-3095}} % 2540
  \author{J.~S.~Lange\,\orcidlink{0000-0003-0234-0474}} % 2277
  \author{M.~Laurenza\,\orcidlink{0000-0002-7400-6013}} % 10223
% \author{K.~Lautenbach\,\orcidlink{0000-0003-3762-694X}} % 2102
% \author{P.~J.~Laycock\,\orcidlink{0000-0002-8572-5339}} % 7683
  \author{R.~Leboucher\,\orcidlink{0000-0003-3097-6613}} % 14083
% \author{F.~R.~Le~Diberder\,\orcidlink{0000-0002-9073-5689}} % 3267
% \author{J.~K.~Lee\,\orcidlink{0000-0001-6397-0723}} % 2190
  \author{M.~J.~Lee\,\orcidlink{0000-0003-4528-4601}} % 21803
% \author{S.~C.~Lee\,\orcidlink{0000-0002-9835-1006}} % 2544
% \author{P.~Leitl\,\orcidlink{0000-0002-1336-9558}} % 2414
  \author{C.~Lemettais\,\orcidlink{0009-0008-5394-5100}} % 22704
  \author{P.~Leo\,\orcidlink{0000-0003-3833-2900}} % 19823
  \author{D.~Levit\,\orcidlink{0000-0001-5789-6205}} % 2507
% \author{P.~M.~Lewis\,\orcidlink{0000-0002-5991-622X}} % 2582
% \author{C.~Li\,\orcidlink{0000-0002-3240-4523}} % 2325
  \author{L.~K.~Li\,\orcidlink{0000-0002-7366-1307}} % 3263
  \author{S.~X.~Li\,\orcidlink{0000-0003-4669-1495}} % 2377
  \author{Y.~Li\,\orcidlink{0000-0002-4413-6247}} % 8083
  \author{Y.~B.~Li\,\orcidlink{0000-0002-9909-2851}} % 2573
  \author{J.~Libby\,\orcidlink{0000-0002-1219-3247}} % 2262
% \author{K.~Lieret\,\orcidlink{0000-0003-2792-7511}} % 2268
% \author{J.~Lin\,\orcidlink{0000-0002-3653-2899}} % 2401
  \author{Z.~Liptak\,\orcidlink{0000-0002-6491-8131}} % 3565
  \author{M.~H.~Liu\,\orcidlink{0000-0002-9376-1487}} % 15244
  \author{Q.~Y.~Liu\,\orcidlink{0000-0002-7684-0415}} % 7045
% \author{Y.~Liu\,\orcidlink{0000-0002-8374-3947}} % 16223
% \author{Z.~A.~Liu\,\orcidlink{0000-0002-2896-1386}} % 3283
  \author{Z.~Q.~Liu\,\orcidlink{0000-0002-0290-3022}} % 11303
  \author{D.~Liventsev\,\orcidlink{0000-0003-3416-0056}} % 2578
  \author{S.~Longo\,\orcidlink{0000-0002-8124-8969}} % 2396
% \author{A.~Lozar\,\orcidlink{0000-0002-0569-6882}} % 12423
  \author{T.~Lueck\,\orcidlink{0000-0003-3915-2506}} % 2406
% \author{T.~Luo\,\orcidlink{0000-0001-5139-5784}} % 3268
  \author{C.~Lyu\,\orcidlink{0000-0002-2275-0473}} % 12484
  \author{Y.~Ma\,\orcidlink{0000-0001-8412-8308}} % 16883
  \author{M.~Maggiora\,\orcidlink{0000-0003-4143-9127}} % 5343
  \author{S.~P.~Maharana\,\orcidlink{0000-0002-1746-4683}} % 19083
  \author{R.~Maiti\,\orcidlink{0000-0001-5534-7149}} % 12043
  \author{S.~Maity\,\orcidlink{0000-0003-3076-9243}} % 2985
  \author{G.~Mancinelli\,\orcidlink{0000-0003-1144-3678}} % 20743
  \author{R.~Manfredi\,\orcidlink{0000-0002-8552-6276}} % 10303
  \author{E.~Manoni\,\orcidlink{0000-0002-9826-7947}} % 2305
% \author{A.~C.~Manthei\,\orcidlink{0000-0002-6900-5729}} % 15023
  \author{M.~Mantovano\,\orcidlink{0000-0002-5979-5050}} % 19783
  \author{D.~Marcantonio\,\orcidlink{0000-0002-1315-8646}} % 11163
  \author{S.~Marcello\,\orcidlink{0000-0003-4144-863X}} % 4223
  \author{C.~Marinas\,\orcidlink{0000-0003-1903-3251}} % 2133
% \author{L.~Martel\,\orcidlink{0000-0001-8562-0038}} % 13503
  \author{C.~Martellini\,\orcidlink{0000-0002-7189-8343}} % 16983
  \author{A.~Martens\,\orcidlink{0000-0003-1544-4053}} % 13823
  \author{A.~Martini\,\orcidlink{0000-0003-1161-4983}} % 2336
  \author{T.~Martinov\,\orcidlink{0000-0001-7846-1913}} % 19463
  \author{L.~Massaccesi\,\orcidlink{0000-0003-1762-4699}} % 16323
  \author{M.~Masuda\,\orcidlink{0000-0002-7109-5583}} % 2238
% \author{T.~Matsuda\,\orcidlink{0000-0003-4673-570X}} % 5543
  \author{K.~Matsuoka\,\orcidlink{0000-0003-1706-9365}} % 2316
  \author{D.~Matvienko\,\orcidlink{0000-0002-2698-5448}} % 2351
  \author{S.~K.~Maurya\,\orcidlink{0000-0002-7764-5777}} % 9763
% \author{F.~Mawas\,\orcidlink{0000-0002-7176-4732}} % 20943
  \author{J.~A.~McKenna\,\orcidlink{0000-0001-9871-9002}} % 2392
% \author{F.~Meggendorfer\,\orcidlink{0000-0002-1466-7207}} % 7103
% \author{R.~Mehta\,\orcidlink{0000-0001-8670-3409}} % 15203
  \author{F.~Meier\,\orcidlink{0000-0002-6088-0412}} % 3103
  \author{M.~Merola\,\orcidlink{0000-0002-7082-8108}} % 2456
  \author{F.~Metzner\,\orcidlink{0000-0002-0128-264X}} % 2296
% \author{M.~Milesi\,\orcidlink{0000-0002-8805-1886}} % 5443
  \author{C.~Miller\,\orcidlink{0000-0003-2631-1790}} % 2273
  \author{M.~Mirra\,\orcidlink{0000-0002-1190-2961}} % 14744
  \author{S.~Mitra\,\orcidlink{0000-0002-1118-6344}} % 19944
  \author{K.~Miyabayashi\,\orcidlink{0000-0003-4352-734X}} % 2327
% \author{H.~Miyake\,\orcidlink{0000-0002-7079-8236}} % 2452
% \author{R.~Mizuk\,\orcidlink{0000-0002-2209-6969}} % 2483
  \author{G.~B.~Mohanty\,\orcidlink{0000-0001-6850-7666}} % 2278
% \author{N.~Molina-Gonzalez\,\orcidlink{0000-0002-0903-1722}} % 8004
  \author{S.~Mondal\,\orcidlink{0000-0002-3054-8400}} % 19743
  \author{S.~Moneta\,\orcidlink{0000-0003-2184-7510}} % 13303
% \author{H.~Moon\,\orcidlink{0000-0001-5213-6477}} % 2304
  \author{H.-G.~Moser\,\orcidlink{0000-0003-3579-9951}} % 2120
  \author{M.~Mrvar\,\orcidlink{0000-0001-6388-3005}} % 2527
% \author{Th.~Muller\,\orcidlink{0000-0003-4337-0098}} % 2165
% \author{R.~Mussa\,\orcidlink{0000-0002-0294-9071}} % 2372
  \author{I.~Nakamura\,\orcidlink{0000-0002-7640-5456}} % 3463
% \author{K.~R.~Nakamura\,\orcidlink{0000-0001-7012-7355}} % 2417
% \author{E.~Nakano\,\orcidlink{0000-0003-2282-5217}} % 2554
% \author{T.~Nakano\,\orcidlink{0000-0003-3157-5328}} % 2983
  \author{M.~Nakao\,\orcidlink{0000-0001-8424-7075}} % 2498
% \author{H.~Nakayama\,\orcidlink{0000-0002-2030-9967}} % 2232
% \author{H.~Nakazawa\,\orcidlink{0000-0003-1684-6628}} % 2335
  \author{Y.~Nakazawa\,\orcidlink{0000-0002-6271-5808}} % 17383
% \author{A.~Narimani~Charan\,\orcidlink{0000-0002-5975-550X}} % 10143
  \author{M.~Naruki\,\orcidlink{0000-0003-1773-2999}} % 4583
  \author{D.~Narwal\,\orcidlink{0000-0001-6585-7767}} % 7223
  \author{Z.~Natkaniec\,\orcidlink{0000-0003-0486-9291}} % 3923
  \author{A.~Natochii\,\orcidlink{0000-0002-1076-814X}} % 12063
% \author{L.~Nayak\,\orcidlink{0000-0002-7739-914X}} % 9464
  \author{M.~Nayak\,\orcidlink{0000-0002-2572-4692}} % 2371
  \author{G.~Nazaryan\,\orcidlink{0000-0002-9434-6197}} % 9523
  \author{M.~Neu\,\orcidlink{0000-0002-4564-8009}} % 23304
% \author{C.~Niebuhr\,\orcidlink{0000-0002-4375-9741}} % 2477
  \author{M.~Niiyama\,\orcidlink{0000-0003-1746-586X}} % 2063
% \author{J.~Ninkovic\,\orcidlink{0000-0003-1523-3635}} % 2386
% \author{N.~K.~Nisar\,\orcidlink{0000-0001-9562-1253}} % 2522
  \author{S.~Nishida\,\orcidlink{0000-0001-6373-2346}} % 2571
% \author{K.~Nishimura\,\orcidlink{0000-0001-8818-8922}} % 3063
% \author{A.~Novosel\,\orcidlink{0000-0002-7308-8950}} % 15523
% \author{K.~Ogawa\,\orcidlink{0000-0003-2220-7224}} % 2430
  \author{S.~Ogawa\,\orcidlink{0000-0002-7310-5079}} % 6263
% \author{S.~L.~Olsen\,\orcidlink{0000-0002-6388-9885}} % 4563
  \author{Y.~Onishchuk\,\orcidlink{0000-0002-8261-7543}} % 2157
  \author{H.~Ono\,\orcidlink{0000-0003-4486-0064}} % 2160
% \author{Y.~Onuki\,\orcidlink{0000-0002-1646-6847}} % 2331
% \author{P.~Oskin\,\orcidlink{0000-0002-7524-0936}} % 9623
% \author{F.~Otani\,\orcidlink{0000-0001-6016-219X}} % 16244
% \author{E.~R.~Oxford\,\orcidlink{0000-0002-0813-4578}} % 6943
% \author{H.~Ozaki\,\orcidlink{0000-0001-6901-1881}} % 2984
% \author{P.~Pakhlov\,\orcidlink{0000-0001-7426-4824}} % 2221
  \author{G.~Pakhlova\,\orcidlink{0000-0001-7518-3022}} % 2188
% \author{A.~Paladino\,\orcidlink{0000-0002-3370-259X}} % 2435
% \author{T.~Pang\,\orcidlink{0000-0003-1204-0846}} % 2114
% \author{A.~Panta\,\orcidlink{0000-0001-6385-7712}} % 7943
% \author{E.~Paoloni\,\orcidlink{0000-0001-5969-8712}} % 2488
  \author{S.~Pardi\,\orcidlink{0000-0001-7994-0537}} % 2532
  \author{K.~Parham\,\orcidlink{0000-0001-9556-2433}} % 10684
  \author{H.~Park\,\orcidlink{0000-0001-6087-2052}} % 2284
  \author{J.~Park\,\orcidlink{0000-0001-6520-0028}} % 18203
  \author{S.-H.~Park\,\orcidlink{0000-0001-6019-6218}} % 2509
  \author{B.~Paschen\,\orcidlink{0000-0003-1546-4548}} % 2159
  \author{A.~Passeri\,\orcidlink{0000-0003-4864-3411}} % 2116
  \author{S.~Patra\,\orcidlink{0000-0002-4114-1091}} % 3123
  \author{S.~Paul\,\orcidlink{0000-0002-8813-0437}} % 2131
  \author{T.~K.~Pedlar\,\orcidlink{0000-0001-9839-7373}} % 2421
% \author{I.~Peruzzi\,\orcidlink{0000-0001-6729-8436}} % 2253
  \author{R.~Peschke\,\orcidlink{0000-0002-2529-8515}} % 7123
  \author{R.~Pestotnik\,\orcidlink{0000-0003-1804-9470}} % 2476
% \author{F.~Pham\,\orcidlink{0000-0003-0608-2302}} % 2963
  \author{M.~Piccolo\,\orcidlink{0000-0001-9750-0551}} % 2147
  \author{L.~E.~Piilonen\,\orcidlink{0000-0001-6836-0748}} % 2346
  \author{G.~Pinna~Angioni\,\orcidlink{0000-0003-0808-8281}} % 13363
  \author{P.~L.~M.~Podesta-Lerma\,\orcidlink{0000-0002-8152-9605}} % 2266
  \author{T.~Podobnik\,\orcidlink{0000-0002-6131-819X}} % 11223
  \author{S.~Pokharel\,\orcidlink{0000-0002-3367-738X}} % 12283
% \author{L.~Polat\,\orcidlink{0000-0002-2260-8012}} % 9783
% \author{V.~Popov\,\orcidlink{0000-0003-0208-2583}} % 2096
  \author{C.~Praz\,\orcidlink{0000-0002-6154-885X}} % 2726
  \author{S.~Prell\,\orcidlink{0000-0002-0195-8005}} % 12743
  \author{E.~Prencipe\,\orcidlink{0000-0002-9465-2493}} % 2219
  \author{M.~T.~Prim\,\orcidlink{0000-0002-1407-7450}} % 2501
  \author{I.~Prudiiev\,\orcidlink{0000-0002-0819-284X}} % 19383
% \author{M.~V.~Purohit\,\orcidlink{0000-0002-8381-8689}} % 2196
  \author{H.~Purwar\,\orcidlink{0000-0002-3876-7069}} % 12363
% \author{A.~Rabusov\,\orcidlink{0000-0001-8189-7398}} % 2355
% \author{N.~Rad\,\orcidlink{0000-0002-5204-0851}} % 11683
  \author{P.~Rados\,\orcidlink{0000-0003-0690-8100}} % 7383
  \author{G.~Raeuber\,\orcidlink{0000-0003-2948-5155}} % 18143
  \author{S.~Raiz\,\orcidlink{0000-0001-7010-8066}} % 13003
  \author{N.~Rauls\,\orcidlink{0000-0002-6583-4888}} % 11603
% \author{K.~Ravindran\,\orcidlink{0000-0002-5584-2614}} % 22503
  \author{M.~Reif\,\orcidlink{0000-0002-0706-0247}} % 8043
  \author{S.~Reiter\,\orcidlink{0000-0002-6542-9954}} % 2248
  \author{M.~Remnev\,\orcidlink{0000-0001-6975-1724}} % 2785
  \author{L.~Reuter\,\orcidlink{0000-0002-5930-6237}} % 16403
  \author{I.~Ripp-Baudot\,\orcidlink{0000-0002-1897-8272}} % 2469
% \author{M.~Ritzert\,\orcidlink{0000-0003-2928-7044}} % 2526
  \author{G.~Rizzo\,\orcidlink{0000-0003-1788-2866}} % 2579
% \author{L.~B.~Rizzuto\,\orcidlink{0000-0001-6621-6646}} % 3746
  \author{S.~H.~Robertson\,\orcidlink{0000-0003-4096-8393}} % 2471
% \author{P.~Rocchetti\,\orcidlink{0000-0002-2839-3489}} % 13763
% \author{D.~Rodr\'{i}guez~P\'{e}rez\,\orcidlink{0000-0001-8505-649X}} % 2176
  \author{M.~Roehrken\,\orcidlink{0000-0003-0654-2866}} % 11883
  \author{J.~M.~Roney\,\orcidlink{0000-0001-7802-4617}} % 2244
% \author{C.~Rosenfeld\,\orcidlink{0000-0003-3857-1223}} % 2082
  \author{A.~Rostomyan\,\orcidlink{0000-0003-1839-8152}} % 2481
  \author{N.~Rout\,\orcidlink{0000-0002-4310-3638}} % 2965
% \author{M.~Rozanska\,\orcidlink{0000-0003-2651-5021}} % 2205
% \author{G.~Russo\,\orcidlink{0000-0001-5823-4393}} % 2388
% \author{D.~Sahoo\,\orcidlink{0000-0002-5600-9413}} % 2110
% \author{Y.~Sakai\,\orcidlink{0000-0001-9163-3409}} % 2175
% \author{D.~A.~Sanders\,\orcidlink{0000-0002-4902-966X}} % 2458
  \author{S.~Sandilya\,\orcidlink{0000-0002-4199-4369}} % 2286
% \author{A.~Sangal\,\orcidlink{0000-0001-5853-349X}} % 2384
  \author{L.~Santelj\,\orcidlink{0000-0003-3904-2956}} % 2185
% \author{T.~Sanuki\,\orcidlink{0000-0002-4537-5899}} % 6783
% \author{P.~Sartori\,\orcidlink{0000-0002-9528-4338}} % 4523
  \author{Y.~Sato\,\orcidlink{0000-0003-3751-2803}} % 5243
  \author{V.~Savinov\,\orcidlink{0000-0002-9184-2830}} % 2292
  \author{B.~Scavino\,\orcidlink{0000-0003-1771-9161}} % 2518
% \author{C.~Schmitt\,\orcidlink{0000-0002-3787-687X}} % 15063
% \author{J.~Schmitz\,\orcidlink{0000-0001-8274-8124}} % 12863
  \author{S.~Schneider\,\orcidlink{0009-0002-5899-0353}} % 16803
  \author{G.~Schnell\,\orcidlink{0000-0002-7336-3246}} % 12204
  \author{M.~Schnepf\,\orcidlink{0000-0003-0623-0184}} % 15683
  \author{K.~Schoenning\,\orcidlink{0000-0002-3490-9584}} % 22023
% \author{J.~Schueler\,\orcidlink{0000-0002-2722-6953}} % 2824
  \author{C.~Schwanda\,\orcidlink{0000-0003-4844-5028}} % 2108
% \author{A.~J.~Schwartz\,\orcidlink{0000-0002-7310-1983}} % 2162
% \author{B.~Schwenker\,\orcidlink{0000-0002-7120-3732}} % 2405
% \author{M.~Schwickardi\,\orcidlink{0000-0003-2033-6700}} % 14743
% \author{R.~Seidl\,\orcidlink{0000-0002-6552-6973}} % 26923
  \author{Y.~Seino\,\orcidlink{0000-0002-8378-4255}} % 2517
  \author{A.~Selce\,\orcidlink{0000-0001-8228-9781}} % 9043
  \author{K.~Senyo\,\orcidlink{0000-0002-1615-9118}} % 2987
  \author{J.~Serrano\,\orcidlink{0000-0003-2489-7812}} % 12124
  \author{M.~E.~Sevior\,\orcidlink{0000-0002-4824-101X}} % 2328
  \author{C.~Sfienti\,\orcidlink{0000-0002-5921-8819}} % 2214
  \author{W.~Shan\,\orcidlink{0000-0003-2811-2218}} % 11943
% \author{M.~Shapkin\,\orcidlink{0000-0002-4098-9592}} % 2460
  \author{C.~Sharma\,\orcidlink{0000-0002-1312-0429}} % 11584
% \author{V.~Shebalin\,\orcidlink{0000-0003-1012-0957}} % 2339
  \author{C.~P.~Shen\,\orcidlink{0000-0002-9012-4618}} % 2464
  \author{X.~D.~Shi\,\orcidlink{0000-0002-7006-6107}} % 18843
% \author{H.~Shibuya\,\orcidlink{0000-0002-0197-6270}} % 2234
  \author{T.~Shillington\,\orcidlink{0000-0003-3862-4380}} % 7983
  \author{T.~Shimasaki\,\orcidlink{0000-0003-3291-9532}} % 16263
  \author{J.-G.~Shiu\,\orcidlink{0000-0002-8478-5639}} % 2412
  \author{D.~Shtol\,\orcidlink{0000-0002-0622-6065}} % 9223
% \author{B.~Shwartz\,\orcidlink{0000-0002-1456-1496}} % 2122
  \author{A.~Sibidanov\,\orcidlink{0000-0001-8805-4895}} % 2419
  \author{F.~Simon\,\orcidlink{0000-0002-5978-0289}} % 2164
  \author{J.~B.~Singh\,\orcidlink{0000-0001-9029-2462}} % 2903
% \author{R.~Sinha\,\orcidlink{-}} % 3423
  \author{J.~Skorupa\,\orcidlink{0000-0002-8566-621X}} % 12523
% \author{K.~Smith\,\orcidlink{0000-0003-0446-9474}} % 2243
  \author{R.~J.~Sobie\,\orcidlink{0000-0001-7430-7599}} % 2472
  \author{M.~Sobotzik\,\orcidlink{0000-0002-1773-5455}} % 8604
  \author{A.~Soffer\,\orcidlink{0000-0002-0749-2146}} % 2217
  \author{A.~Sokolov\,\orcidlink{0000-0002-9420-0091}} % 2521
% \author{Y.~Soloviev\,\orcidlink{0000-0003-1136-2827}} % 2479
  \author{E.~Solovieva\,\orcidlink{0000-0002-5735-4059}} % 2398
  \author{S.~Spataro\,\orcidlink{0000-0001-9601-405X}} % 2117
  \author{B.~Spruck\,\orcidlink{0000-0002-3060-2729}} % 2493
% \author{S.~Stani\v{c}\,\orcidlink{0000-0003-3344-8381}} % 3383
  \author{M.~Stari\v{c}\,\orcidlink{0000-0001-8751-5944}} % 2326
  \author{P.~Stavroulakis\,\orcidlink{0000-0001-9914-7261}} % 20643
  \author{S.~Stefkova\,\orcidlink{0000-0003-2628-530X}} % 8783
% \author{Z.~S.~Stottler\,\orcidlink{0000-0002-1898-5333}} % 2267
  \author{R.~Stroili\,\orcidlink{0000-0002-3453-142X}} % 2465
% \author{J.~Strube\,\orcidlink{0000-0001-7470-9301}} % 2451
  \author{Y.~Sue\,\orcidlink{0000-0003-2430-8707}} % 2085
% \author{R.~Sugiura\,\orcidlink{0000-0002-6044-5445}} % 4644
  \author{M.~Sumihama\,\orcidlink{0000-0002-8954-0585}} % 4243
% \author{K.~Sumisawa\,\orcidlink{0000-0001-7003-7210}} % 2583
% \author{W.~Sutcliffe\,\orcidlink{0000-0002-9795-3582}} % 3784
  \author{N.~Suwonjandee\,\orcidlink{0009-0000-2819-5020}} % 14063
% \author{S.~Y.~Suzuki\,\orcidlink{0000-0002-7135-4901}} % 2496
  \author{H.~Svidras\,\orcidlink{0000-0003-4198-2517}} % 11783
% \author{M.~Tabata\,\orcidlink{0000-0001-6138-1028}} % 2986
% \author{M.~Takahashi\,\orcidlink{0000-0003-1171-5960}} % 2467
  \author{M.~Takizawa\,\orcidlink{0000-0001-8225-3973}} % 2437
  \author{U.~Tamponi\,\orcidlink{0000-0001-6651-0706}} % 2366
% \author{S.~Tanaka\,\orcidlink{0000-0002-6029-6216}} % 2530
  \author{K.~Tanida\,\orcidlink{0000-0002-8255-3746}} % 3803
% \author{H.~Tanigawa\,\orcidlink{0000-0003-3681-9985}} % 2237
% \author{N.~Taniguchi\,\orcidlink{0000-0002-1462-0564}} % 2285
  \author{F.~Tenchini\,\orcidlink{0000-0003-3469-9377}} % 2546
% \author{Y.~Teramoto\,\orcidlink{0000-0002-1738-6697}} % 26063
  \author{A.~Thaller\,\orcidlink{0000-0003-4171-6219}} % 16044
  \author{O.~Tittel\,\orcidlink{0000-0001-9128-6240}} % 8663
  \author{R.~Tiwary\,\orcidlink{0000-0002-5887-1883}} % 10403
  \author{D.~Tonelli\,\orcidlink{0000-0002-1494-7882}} % 4564
  \author{E.~Torassa\,\orcidlink{0000-0003-2321-0599}} % 2556
% \author{N.~Toutounji\,\orcidlink{0000-0002-1937-6732}} % 2263
  \author{K.~Trabelsi\,\orcidlink{0000-0001-6567-3036}} % 2369
% \author{I.~Tsaklidis\,\orcidlink{0000-0003-3584-4484}} % 13443
% \author{T.~Tsuboyama\,\orcidlink{0000-0002-4575-1997}} % 2361
% \author{N.~Tsuzuki\,\orcidlink{0000-0003-1141-1908}} % 2352
% \author{M.~Uchida\,\orcidlink{0000-0003-4904-6168}} % 2370
  \author{I.~Ueda\,\orcidlink{0000-0002-6833-4344}} % 2519
% \author{S.~Uehara\,\orcidlink{0000-0001-7377-5016}} % 2586
% \author{Y.~Uematsu\,\orcidlink{0000-0002-0296-4028}} % 5883
  \author{T.~Uglov\,\orcidlink{0000-0002-4944-1830}} % 2252
  \author{K.~Unger\,\orcidlink{0000-0001-7378-6671}} % 9463
  \author{Y.~Unno\,\orcidlink{0000-0003-3355-765X}} % 2420
  \author{K.~Uno\,\orcidlink{0000-0002-2209-8198}} % 14963
  \author{S.~Uno\,\orcidlink{0000-0002-3401-0480}} % 2149
% \author{P.~Urquijo\,\orcidlink{0000-0002-0887-7953}} % 2302
  \author{Y.~Ushiroda\,\orcidlink{0000-0003-3174-403X}} % 2317
% \author{Y.~V.~Usov\,\orcidlink{0000-0003-3144-2920}} % 5003
  \author{S.~E.~Vahsen\,\orcidlink{0000-0003-1685-9824}} % 2251
  \author{R.~van~Tonder\,\orcidlink{0000-0002-7448-4816}} % 2706
% \author{G.~S.~Varner\,\orcidlink{0000-0002-0302-8151}} % 2119
  \author{K.~E.~Varvell\,\orcidlink{0000-0003-1017-1295}} % 2545
  \author{M.~Veronesi\,\orcidlink{0000-0002-1916-3884}} % 20723
  \author{A.~Vinokurova\,\orcidlink{0000-0003-4220-8056}} % 2289
  \author{V.~S.~Vismaya\,\orcidlink{0000-0002-1606-5349}} % 16063
  \author{L.~Vitale\,\orcidlink{0000-0003-3354-2300}} % 2415
  \author{V.~Vobbilisetti\,\orcidlink{0000-0002-4399-5082}} % 7364
  \author{R.~Volpe\,\orcidlink{0000-0003-1782-2978}} % 20183
% \author{V.~Vorobyev\,\orcidlink{0000-0002-6660-868X}} % 2298
  \author{A.~Vossen\,\orcidlink{0000-0003-0983-4936}} % 2249
  \author{B.~Wach\,\orcidlink{0000-0003-3533-7669}} % 8203
% \author{E.~Waheed\,\orcidlink{0000-0001-7774-0363}} % 2226
  \author{M.~Wakai\,\orcidlink{0000-0003-2818-3155}} % 3583
% \author{H.~M.~Wakeling\,\orcidlink{0000-0003-4606-7895}} % 3664
  \author{S.~Wallner\,\orcidlink{0000-0002-9105-1625}} % 20363
% \author{W.~Wan~Abdullah\,\orcidlink{0000-0001-5798-9145}} % 2280
% \author{B.~Wang\,\orcidlink{0000-0001-6136-6952}} % 2569
% \author{C.~H.~Wang\,\orcidlink{0000-0001-6760-9839}} % 2224
  \author{E.~Wang\,\orcidlink{0000-0001-6391-5118}} % 10983
  \author{M.-Z.~Wang\,\orcidlink{0000-0002-0979-8341}} % 2074
  \author{X.~L.~Wang\,\orcidlink{0000-0001-5805-1255}} % 2076
  \author{Z.~Wang\,\orcidlink{0000-0002-3536-4950}} % 15743
  \author{A.~Warburton\,\orcidlink{0000-0002-2298-7315}} % 2347
% \author{M.~Watanabe\,\orcidlink{0000-0001-6917-6694}} % 2309
  \author{S.~Watanuki\,\orcidlink{0000-0002-5241-6628}} % 6843
% \author{M.~Welsch\,\orcidlink{0000-0002-3026-1872}} % 7023
% \author{O.~Werbycka\,\orcidlink{0000-0002-0614-8773}} % 6123
  \author{C.~Wessel\,\orcidlink{0000-0003-0959-4784}} % 2100
% \author{J.~Wiechczynski\,\orcidlink{0000-0002-3151-6072}} % 2604
% \author{P.~Wieduwilt\,\orcidlink{0000-0002-1706-5359}} % 2343
% \author{H.~Windel\,\orcidlink{0000-0001-9472-0786}} % 2081
  \author{E.~Won\,\orcidlink{0000-0002-4245-7442}} % 2410
  \author{Y.~Xie\,\orcidlink{0000-0002-0170-2798}} % 20383
  \author{X.~P.~Xu\,\orcidlink{0000-0001-5096-1182}} % 4923
  \author{B.~D.~Yabsley\,\orcidlink{0000-0002-2680-0474}} % 3645
  \author{S.~Yamada\,\orcidlink{0000-0002-8858-9336}} % 2492
% \author{H.~Yamamoto\,\orcidlink{-}} % 2964
  \author{W.~Yan\,\orcidlink{0000-0003-0713-0871}} % 2094
  \author{S.~B.~Yang\,\orcidlink{0000-0002-9543-7971}} % 2374
  \author{J.~Yelton\,\orcidlink{0000-0001-8840-3346}} % 2067
  \author{J.~H.~Yin\,\orcidlink{0000-0002-1479-9349}} % 2365
  \author{Y.~M.~Yook\,\orcidlink{0000-0002-4912-048X}} % 2453
  \author{K.~Yoshihara\,\orcidlink{0000-0002-3656-2326}} % 12663
  \author{C.~Z.~Yuan\,\orcidlink{0000-0002-1652-6686}} % 2088
  \author{Y.~Yusa\,\orcidlink{0000-0002-4001-9748}} % 2357
  \author{L.~Zani\,\orcidlink{0000-0003-4957-805X}} % 2529
  \author{F.~Zeng\,\orcidlink{0009-0003-6474-3508}} % 22043
  \author{B.~Zhang\,\orcidlink{0000-0002-5065-8762}} % 11663
% \author{J.~Z.~Zhang\,\orcidlink{0000-0001-6535-0659}} % 2349
% \author{Y.~Zhang\,\orcidlink{0000-0003-2961-2820}} % 3303
% \author{Z.~Zhang\,\orcidlink{0000-0001-6140-2044}} % 5363
  \author{V.~Zhilich\,\orcidlink{0000-0002-0907-5565}} % 4703
  \author{J.~S.~Zhou\,\orcidlink{0000-0002-6413-4687}} % 12463
  \author{Q.~D.~Zhou\,\orcidlink{0000-0001-5968-6359}} % 7323
% \author{X.~Y.~Zhou\,\orcidlink{0000-0002-0299-4657}} % 2380
  \author{V.~I.~Zhukova\,\orcidlink{0000-0002-8253-641X}} % 2387
% \author{V.~Zhulanov\,\orcidlink{0000-0002-0306-9199}} % 4983
  \author{R.~\v{Z}leb\v{c}\'{i}k\,\orcidlink{0000-0003-1644-8523}} % 13403
\collaboration{The Belle and Belle II Collaborations}

